Towards Language Models That Can See: Computer Vision Through the LENS of Natural Language

We propose LENS, a modular approach for tackling computer vision problems by leveraging the power of large language models (LLMs). Our system uses a language model to reason over outputs from a set of independent and highly descriptive vision modules that provide exhaustive information about an image. We evaluate the approach on pure computer vision settings such as zero- and few-shot object recognition, as well as on vision and language problems. LENS can be applied to any off-the-shelf LLM and we find that the LLMs with LENS perform highly competitively with much bigger and much more sophisticated systems, without any multimodal training whatsoever. We open-source our code at https://github.com/ContextualAI/lens and provide an interactive demo.

==> Figures/comparison.tex <==
\begin{figure*}[t]
  \centering
  \includegraphics[width=1\textwidth]{Files/incorrect_cases.pdf}
  \label{fig:comparison}
  \caption{Comparison between the two approaches for performing fine-grained classification and Vision \& Language using LLMs where the blue blocks represent frozen and the red one represents tunable. Specifically, (a) represents multimodal pre-training and (b) our approach that does not add any additional fine-tuning stage.}
\end{figure*}

==> Tables/ablation_vision_extended.tex <==
\begin{table}
\centering
\begin{tabular}{|c|c|c|c|c|}
\toprule
Dataset    & Attributes & Objects - Attributes & CLIP - ZS\\
\midrule 
Pets       & 91.0 & 92.6 & 90.1 \\
DTD        & 51.5 & 57.8 & 53.7\\
Aircraft   & 36.5 & 38.5 & 38 \\
Caltech101 & 71.6 & 75.4 & 75.6\\
Flowers102 & 75.6 & 76.6 & 74.9\\
Food101    & 89.12 & 90.8 & 92.6\\
Cars       & 92.1 & 92.9 & 93.4\\
Cifar10    & 93.4 & 95.7 & 95.6\\
ImageNet   & 71.5 & 73.0 & 75.6\\
\midrule 
\textbf{Average} & 74.7 & 77.0 & 76.6 \\
\bottomrule

\end{tabular}
\label{table:hatefulmemes-prompt}
\caption{Fine-grained vision classification ablations. Ablations using clip-tags, attributes and T5Flan-xl}
\label{tab:vision-ablation-extended}
\end{table}

==> Tables/vision_few_shot.tex <==
\begin{table*}[!h]
 \label{tab:vision-zero-few}
 \scriptsize
 \centering
 \begin{tabular}{cccccccccccccc}
 \toprule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Oxford Pets} & \multicolumn{4}{c}{Flowers102} & \multicolumn{4}{c}{FGVC}\\
 \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 \multicolumn{2}{c}{} & CLIP & \multicolumn{3}{c}{Ours} & CLIP & \multicolumn{3}{c}{Ours}  & CLIP & \multicolumn{3}{c}{Ours}\\
 \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} \cmidrule{8-10} \cmidrule(lr){11-11} \cmidrule{12-14}
 Visual Encoder & LLM & 0 & 0 & 1 & 3 & 0 & 0 & 1 & 3 & 0 & 0 & 1 & 3  \\ 
 \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} \cmidrule(lr){8-10} \cmidrule(lr){11-11} \cmidrule(lr){12-14}
 ViT-L/14 & FlanT5\textsubscript{XXL} & 87.8 & 92.0 & 92.1 & 92.6 & 75.5 & 76.4 & 81.6 & 83.0  & 29.5 & 30.1 & 40.8 & 42.1\\
 ViT-L/14 & FlanT5\textsubscript{XL} & 87.8 & 90.1 & 92.0 & 92.2 & 75.5 & 73.0 & 82.7 & 84.0  & 29.5 & 31.1 & 41.1 & 40.4\\
 ViT-H/14 & FlanT5\textsubscript{XXL} & 90.1 & 92.4 & 92.8 & 93.1 & 74.9 & 76.7 & 82.3 & 83.8  & 37.97 & 38.5 & 48.5 & 48.1\\
 ViT-H/14 & FlanT5\textsubscript{XL} & 90.1 & 92.6 & 92.4 & 92.7 & 74.9 & 76.6 & 83.7 & 85.0  & 37.97 & 38.5 & 48.4 & 49.3\\

 \midrule\midrule
 \multicolumn{2}{c}{} & \multicolumn{4}{c}{Caltech101} & \multicolumn{4}{c}{Food101} & \multicolumn{4}{c}{DTD} \\
 \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14}
 \multicolumn{2}{c}{} & CLIP & \multicolumn{3}{c}{Ours} & CLIP & \multicolumn{3}{c}{Ours}  & CLIP & \multicolumn{3}{c}{Ours}\\
 \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} \cmidrule{8-10} \cmidrule(lr){11-11} \cmidrule{12-14}

 Visual Encoder & LLM & 0 & 0 & 1 & 3 & 0 & 0 & 1 & 3 & 0 & 0 & 1 & 3  \\
 \cmidrule(lr){1-1} \cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-6} \cmidrule(lr){7-7} \cmidrule(lr){8-10} \cmidrule(lr){11-11} \cmidrule(lr){12-14}
 ViT-L/14 & FlanT5\textsubscript{XXL} & 70.4 & 71.9 & 76.9 & 81.1 & 89.8 & 91.6 & 91.5 & 91.4 & 50.7 & 49.0 & 58.8 & 61.3\\
 ViT-L/14 & FlanT5\textsubscript{XL} & 70.4 & 71.3 & 78.9 & 80.2 & 89.8 & 90.1 & 92.1 & 92.3 & 50.7 & 47.6 & 58.1 & 58.1\\

 ViT-H/14 & FlanT5\textsubscript{XXL} & 75.6 & 75.5 & 80.1 & 82.3 & 92.6 & 91.7 & 90.8 & 90.7 & 53.7 & 58.5 & 64.6 & 66.2\\
 ViT-H/14 & FlanT5\textsubscript{XL} & 75.6 & 75.4 & 81.8 & 82.8 & 92.6 & 89.4 & 91.5 & 91.9 & 53.7 & 57.8 & 63.8 & 63.6 \\

 \toprule
 \end{tabular}%
 \caption{Zero and few shot evaluation of \modelName. Experiments demonstrated the effectiveness of LLM in solving fine-grained classification tasks leveraging text information provided by ``vision modules"}

 \end{table*}

